Pooling-Invariant Image Feature Learning

Unsupervised dictionary learning has been a key component in state-of-the-art computer vision recognition architectures. While highly effective methods exist for patch-based dictionary learning, these methods may learn redundant features after the pooling stage in a given early vision architecture. In this paper, we offer a novel dictionary learning scheme to efficiently take into account the invariance of learned features after the spatial pooling stage. The algorithm is built on simple clustering, and thus enjoys efficiency and scalability. We discuss the underlying mechanism that justifies the use of clustering algorithms, and empirically show that the algorithm finds better dictionaries than patch-based methods with the same dictionary size.

==> include/algorithm-old.tex <==
\section{Feature Learning from a Nystr\"{o}m Perspective}
Unsupervised feature learning with a single layer has been extensively explored in the recent literature. An especially interesting finding is that for a single layer, naive approaches such as k-means and orthogonal matching pursuit (OMP) shows a surprisingly high performance when coupled with non-linear feedforward encoding approaches \cite{Coates}. Moreover, randomly sampled or generated filters are also shown to perform well \cite{somepaper}. In this section, we first propose to view the single layer feature learning as a matrix approximation problem, and then use theoretical results from Nystr\"{o}m sampling to show that a theoretical limitation exists in a single layer structure: as the codebook grows larger, the effectiveness of adding new codes diminishes following a power law. \note{is this name appropriate?}.

\todo{write the Nystrom story}

\section{Learning Unsupervised Features with Budgeted Codebooks}
In additional to the theoretical bound presented above, another practical issue in image classification is that it's computationally prohibitive to use large dictionaries. This is especially true when we have more than 1 layer of feature extraction, as a large convolutional layer would immediately drive up the number of parameters in the next layer. Thus, learning a codebook that is under a certain budget while still keeps useful information would be necessary. We first give a brief review of the feature extraction pipeline we adopted.

\subsection{Feature Extraction Pipeline}

\subsection{Greedy Budgeted Codebook Learning}
As the codebook learning method we adopted is efficient and scalable, it is relatively easy to learn a large codebook pro tempore when we train a single layer. Back to the Nystr\"{o}m theory, this gives us a good approximation of the ideal encoding result given by the current layer. Our goal is then to select a subset of the codebook so that when we encode the features with the reduced codebook, the information contained in the encoded results with the larger codebook is best preserved.

We formulate the codebook selection problem as an information gain maximization problem. Specifically, denote the encoded feature vector using the original codebook $\bD$ by $\bx_{D}$, and the encoded feature vector using a subset codebook $\bS \subset \bD$ by $\bx_{S}$, the conditional entropy of $\bx_{D}$ given $\bx_{S}$ could be written as
\begin{equation}
    H(\bx_{D}|\bx_{S}) = -\int_{\bx_{D}} P(\bx_{D}) \log(\bx_{D}|\bx_{S}).
\end{equation}

To this end, we make an assumption \note{do we need to justify it? While the distribution of image features are often non-Gaussian, many algorithms such as sparse coding often still aim to minimize the L2 error, effectively imposing a Gaussian noise assumption} that the encoded features follow a Gaussian distribution, for which the differential entropy provides a good measure of information / uncertainty. 
For Gaussian distributions, the conditional entropy could be computed with the covariance matrix as:
\begin{equation}
    H(\bx_{D}|\bx_{S}) = \frac{1}{2}\ln(\det(\Sigma_{\bx_{D}})) + \frac{N}{2}\ln(2\pi e)
\end{equation}

The general problem of maximizing the 

In addition, notice that the pooling stage yields the same feature dimension for each pooling region as the encoded features has, so the feature selection algorithm could be carried out after the pooling stage to also take advantage of the spatial invariance.


\subsection{Related Work}
\todo{discuss Adam Coates' work?}
\subsection{Exemplar Results}
